Succinct Dynamic Ordered Sets with Random Access

The representation of a dynamic ordered set of $n$ integer keys drawn from a universe of size $m$ is a fundamental data structuring problem. Many solutions to this problem achieve optimal time but take polynomial space, therefore preserving time optimality in the \emph{compressed} space regime is the problem we address in this work. For a polynomial universe $m = n^{\Theta(1)}$, we give a solution that takes $\textsf{EF}(n,m) + o(n)$ bits, where $\textsf{EF}(n,m) \leq n\lceil \log_2(m/n)\rceil + 2n$ is the cost in bits of the \emph{Elias-Fano} representation of the set, and supports random access to the $i$-th smallest element in $O(\log n/ \log\log n)$ time, updates and predecessor search in $O(\log\log n)$ time. These time bounds are optimal.

==> extension.tex <==
\section{Non-polynomial universes}\label{sec:non_polynomial}

In this section, we show how to handle
\emph{non-polynomial} universes.
In this (more) general case, the lower bound for dynamic predecessor search
is $O(\log_w n) = O(\log n / \log\log m)$ that corresponds to the first branch
of the time/space trade-off from Theorem~\ref{thm:pred},
as well as the one for {\access}, {\ins} and {\del}~\cite{PT14}.

\return
Before proceeding, we make the following observation.
The data structure of Theorem~\ref{thm:dynamic_opt_ef1}
allows us to support all operations in time $O(\log\log m)$
when non-polynomial universes are considered.
In this case, the data structure of Lemma~\ref{lem:small_blocks_ds}
will take $O(\polylg m \log\log m)$ bits and operate in $O(\log\log m)$ time. In order to guarantee an overall redundancy of $o(n)$ bits, we let mini blocks be of size $\Theta((\log\log m)^2)$ and group $O(\log^2 m)$ consecutive mini blocks into a block.
The high part of a mini block fits into one machine word, whereas we can insert/delete a low part in $O((\log\log m)^{2\epsilon})$ for Lemma~\ref{lem:dynamic_array}, which is $O(\log\log u)$ as soon as $\epsilon < 1/2$.
The following corollary matches the asymptotic time bounds of $y$-fast tries and van Emde Boas trees but in almost optimally compressed space.

\begin{cor}
An ordered set $\seq \subseteq \{0,\ldots,m\}$,
with $|\seq| = n$, can be represented in
$\ef(n,m) + o(n)$ bits
such that
{\access} and {\pred} are supported in $O(\log\log m)$ worst-case,
{\ins}/{\del} in $O(\log\log m)$ expected time.
\end{cor}

\return
In the rest of this section, we will show the following theorem instead.

\begin{thm}\label{thm:dynamic_opt_ef2}
An ordered set $\seq \subseteq \{0,\ldots,m\}$,
with $|\seq| = n$, can be represented in
$O(\ef(n,m) + n)$ bits
such that
{\access} and {\pred} is supported in $O(\log n / \log w)$ worst-case,
{\ins}/{\del} in $O(\log n / \log w)$ amortized time.
\end{thm}

%Notice that the results in Theorem~\ref{thm:dynamic_opt_ef2} occupies $O(1)$
%bits more per integer with respect to the static Elias-Fano space bound,
%against the $o(1)$-bit overhead exhibited in Theorem~\ref{thm:dynamic_opt_ef1}.
%(and also Theorem~\ref{thm:static} and~\ref{thm:ext_ef}).

%Our approach will follow a standard reduction due to~\citet*{Willard00},
%captured with the following lemma.
%
%\begin{lem}{\textup{\citet*{Willard00}}}\label{lem:willard}
%A leaf-oriented $B$-tree with out-degree $B$ and height $h$
%can be maintained in $O(h)$ worst-case time if:
%searches, insertions and deletions take $O(1)$ time per node when no splits or merges occur, and
%merging or splitting a node of size $B$ requires $O(B)$ time.
%\end{lem}
%
%
%Therefore, we first describe a solution for a small set of integers,
%namely $n = w^{O(1)}$, supporting the operations in $O(1)$ time.
%Then, embedding this data structure for small sets in the nodes of a
%weight-balanced $B$-tree with branching factor $B = w^{O(1)}$ yields a data structure supporting the mentioned operations in $O(\log_w n)$ time~\cite{RRR01,DP04,PT14,Dietz89,Willard00}.


\subsection{Small sets}

We show the following lemma.

\begin{lem}\label{lem:small_sets_compressed}
An ordered set $\seq \subseteq \{0,\ldots,m\}$,
with $|\seq| = n = w^{O(1)}$, can be represented in
$O(\ef(n,m)) + 2n$ bits and supporting
{\access} and {\pred} in $O(1)$ worst-case,
{\ins} and {\del} in $O(1)$ amortized time.
\end{lem}

%\parag{Data structure and space analysis}
\begin{proof}
We represent the set $\seq$ with Elias-Fano. The high part of the Elias-Fano representation of $\seq$ is made by a bitvector $H$ of at most $2n = \Oh(w)$ bits which fits in a machine word and is operated in $\Oh(1)$ time.
The low part is instead an \emph{unsorted} vector $L$ of size $n = w^{\Oh(1)}$, whose integers require $\lceil\log(m/n)\rceil$ bits each.

What we need is a representation of $L$ that supports the wanted operations in $\Oh(1)$ time.
We proceed as follows. We divide $L$ in its $s \leq n$ \emph{sorted runs} $L_1,\ldots,L_s$, each run comprising all the low parts of the integers of $\seq$ that share the same high part, i.e., whose $\lceil \log n \rceil$ most significant bits are the same. Each sorted run $L_i$ is represented with
the \emph{dynamic fusion node} data structure of Lemma~\ref{lem:small_sets}.
The space required by $L$ is therefore $O(n\log(m/n))$ bits.
To guarantee that the space of representation of $L$ is bounded by $\Oh(n\log(m/n))$ bits, we rebuild the whole data structure each time the value $\lceil \log(m/n)\rceil$ changes due to insertions/deletions. Since this value changes only a logarithmic number of times for any sequence of operations and we can rebuild the data structure in linear time, a simple amortization argument shows that we can upper bound the cost to $\Oh(1)$ per operation.

%This data structure is depicted in Figure~\ref{fig:small_set}.

%\begin{figure}
%	\centering
%  	\subfloat[]{
%    \includegraphics[scale=0.9]{{{figures/small_set}}}
%    \label{fig:small_set}}
%   	\subfloat[]{
%    \includegraphics[scale=0.8]{{{figures/node}}}
%    \label{fig:node}}
%  	\caption{The left part (a) of the figure illustrates the compressed data structure for small sets. The thick black lines decompose a set of $w^{\Oh(1)}$ integers into $s$ sorted runs of low parts. The instance of the data structure of~\citet*{PT14} storing the low parts belonging to each sorted run is depicted as a triangle, operating in $\Oh(1)$ time.
%  	The right part (b) of the figure shows, instead, an example of tree hierarchy transformation. The gray dots represent the keys of the tree (stored in the leaves), whereas the white dots represent the redundant lower bounds of the sets. The transformation is obtained by removing the redundancy, i.e., by moving the lower bounds of the sets up to the parent node (as indicated by the dashed arrows).}
%\end{figure}

%\parag{Operations}
\return
Now we describe how the operations are implemented.
We reuse part of the description (and notation) of the algorithms for
{\access} and {\pred} described in Section~\ref{sec:ef}.

%In particular, we indicate with $h_x$ and $\ell_x$ the high and low part of a given integer $x$, so that:
%$h_x = x >> \ell$ and $\ell_x = x \, \&\& \, ((1 << \ell) - 1)$, where $\ell = \lceil\log(m/n)\rceil$ is the number of bits needed for the encoding of the average gap of $\seq$. These quantities are calculated in $\Oh(1)$, as well as the re-linking of high and low parts together: $x = (h_x << \ell) \, | \, \ell_x$.
%($\&\&$ stands for the bitwise AND, $|$ for the bitwise OR.)

To support $\access(i)$, we first retrieve the high part $h_i$ of the $i$-th integer as usual, i.e., by following (first part of) the $\access$ algorithm of Elias-Fano (see Section~\ref{sec:ef}).
Then we retrieve the low part of the integer by accessing (through a $\select$ operation, given that the integers in each run are sorted) the value stored at position $p = \rank_1(i) - \rank_1(\select_0(h_i))$ from $L_{h_i}$.
The quantity $p$ is computed on bitvector $H$ in constant time. Notice, in particular, that $\rank_1(\select_0(h_i))$ represents the number of integers of $\seq$ having high part equal to $h_i - 1$. We finally re-link together the retrieved high and low parts.

For the query $\pred(x)$, the problem reduces to determining
$\pred(\ell_x)$ from the integers stored in $L_{h_x}$, which is done in constant time. Re-linking between high and low parts is needed as usual.

To $\ins / \del$ the integer $x$, we first determine $j = \rank_1(\select_0(h_x))$. Then we determine the position of $\ell_x$ within the integers of $L_{h_x}$ by answering a $\rank$ query. Now we know that $x$ is occurring in $\seq$ at position $j + \rank(\ell_x)$ and we can $\ins / \del$ a bit in $H$ at this position in $\Oh(1)$ by using a few machine word operations. Then we finally $\ins / \del$ the low part $\ell_x$ in/from $L_{h_x}$. Each step of the algorithm takes $\Oh(1)$ time.
\end{proof}

%\parag{Note}
%Using the described representation, we also reduce the space of the dynamic prefix sums data structure described in Theorem $6$ of~\cite{BCGSVV15}, since it uses the dynamic fusion node of~\cite{PT14}, whose space has been improved with Lemma~\ref{lem:small_sets_compressed}.
%Such structure supports dynamic prefix sums in $\Oh(1)$ for sets up to $\Oh(w)$ integers. We will also use this result in the following.

\subsection{Final Result}
As already anticipated with Lemma~\ref{lem:willard}, we obtain a solution working for sets of arbitrary size by embedding the data structure of Lemma~\ref{lem:small_sets_compressed} in the nodes of a weight-balanced $B$-tree with branching factor $B = w^{\Oh(1)}$.
%The keys of $\seq$ are stored in the leaves as Elias-Fano compressed blocks of size $\Theta(B) = \rho B$, with $\frac{1}{2} \leq \rho \leq 2$.
The keys of $\seq$ are stored in the leaves of the tree in blocks of size $B$ that are also maintained using the data structure of Lemma~\ref{lem:small_sets_compressed}.
The weight of a node is defined as the number of keys indexed in its sub-tree~\cite{DP04,PT14,Dietz89}.
In particular, each node of the tree stores the lower bounds and sizes of the small sets (up to the leaves) indexed in its sub-tree.
%For the sizes of the sets, we use the dynamic prefix sum data structure of Theorem $6$ of~\cite{BCGSVV15}.
Since for each set stored in an internal node we know its lower bound (as stored in the set of its parent node), the set is re-mapped relatively to its universe of representation because we can subtract the lower bound to all its elements.
Each block of $B$ keys consumes $O(B \log(m/B)) + 2B$ bits
and the keys are remapped relatively to the universe of the block.
Therefore, Property~\ref{prop:almost_convexity} guarantees that the space of representation is bounded by $O(n\log(m/n)) + 2n = O(\ef(n,m))$ bits.

\todo{we have not explained how to support access, i.e.,
how to maintain the sizes of the nodes. we can proceed as explained
in PT14, adopting the trick by patrascu and demaine.
Let $B = w^{O(1)}$.
Therefore, we can use the solution in PT14 in the upper part of the
data structure, for $O(n/B)$ keys, thus taking
$O(n)$ bits overall.
The leaves of the tree store the keys, in blocks of size $B$,
using the data structure of Lemma 8, thus taking
$O(\ef(n,m))$ bits overall. We do not have to store any size information
in the leaves.
In conclusion the space of the data structure is: $O(\ef(n,m) + n)$ bits.}

Lastly, all operations are supported in time $O(\log_w n)$
for Lemma~\ref{lem:willard}.
This concludes the proof of Theorem~\ref{thm:dynamic_opt_ef2}.

%Doing so, the first element of the re-mapped set is always $0$ and, therefore, not represented at all. Refer to Figure~\ref{fig:node} for a pictorial example.
%This applies recursively at each level of the tree, implying that the tree contains \emph{exactly} the $n$ keys of $\seq$ without replication, as in a traditional $B$-tree.
%
%We now aim at showing that such \emph{spreading} of the lower bounds across the levels of the tree introduces an extra space cost, with respect to $\ef(n,m)(\seq(n,u))$, that can be safely bounded with $o(n)$ bits.
%
%For the proof, it is sufficient to consider the deepest internal nodes (branching out to the leaves), given that the upper levels contribute to lower-order terms to the space of the tree.
%Now, consider a node that stores the $k-1$ lower bounds of $k$ leaves, which contain $m$ keys overall. Again refer to Figure~\ref{fig:node}, which is an example for $B=5$ and $k=3$.
%The space of representation of the node is, for Lemma~\ref{lem:small_set}, $\Oh((k-1)\log\frac{u}{k-1}) + 2(k-1) = \Oh(k\log\frac{u}{k}) + 2k$ bits, while the leaves take overall, for Property~\ref{prop:almost_convexity}, at most $(m-k)\lceil\log\frac{u}{m-k}\rceil+2(m-k)$ bits.
%The sum of these two contributions is $m\lceil\log\frac{u}{m-k}\rceil + \Oh(k\log\frac{m-k}{k}) + 2m$ bits.
%We want to show that this quantity is only slightly larger than the bound of $m\lceil\log\frac{u}{m}\rceil+2m$ bits, which is the (static) Elias-Fano encoding of the leaves.
%In fact, the difference between the two quantities is $m\lceil\log\frac{m}{m-k}\rceil + \Oh(k\log\frac{m-k}{k})$, which is independent from the universe $u$ of representation.
%
%\todo{The problem here is that there is actually a dependence on $u$: the difference will be $k(c-1)\log u$, where $c$ is a constant. We should require $c=1$, i.e., the data structure of Lemma 3 requiring exactly $n\log(u/n) + 2n$ bits.
%This idea can be reused for the practical implementation, given that the keys will be encoded with plain EF and $c$ would be exactly 1. This is useful to show a space usage guarantee of the practical implementation.}
%
%It is easy to see that this last formula can be actually rewritten (by adding and subtracting a $\Oh(k\log\frac{m}{m-k})$ term) as $\Oh(k\log\frac{m}{k}+(m-k)\log\frac{m}{m-k})$, which is nothing but $\Oh(mH_0)$, where $H_0$ is the $0$-th order entropy of a source emitting two symbols with empirical probabilities $\frac{k}{m}$ and $\frac{m-k}{m}$ respectively.
%As it is well known, $mH_0$ is a symmetric function and we can restrict our attention to the values of $k$ in $[0, \frac{m}{2})$, obtaining that $mH_0 \approx k\log\frac{m}{k} + k\log e$ bits. Since we have $m$ keys, the loss per the element is therefore $\Oh(H_0) = \Oh(\frac{k}{m}\log\frac{e m}{k}) = \Oh(\log(eB) / B) = o(1)$ bits for \emph{any} choice of $B$ that is $\omega(1)$, given that $m = \Theta(kB)$.
%In what follows, we fix $B$ to be $\log_w n$.
%
%The operations are implemented by traversing the tree in $\Oh(\log_w n)$ time to reach the proper leaf. Then the operation proceeds in the identified leaf, i.e., by accessing an element in $\Oh(1)$ for $\access$; rebuilding the leaf in $\Theta(\log n / \log w)$ for $\ins / \del$; resolving a $\pred / \suc$ query in $\Oh(\log B)$ time with binary search.

%, which generalizes the ones of Theorems~\ref{thm:static_ef_opt_succ},~\ref{thm:ext_ef} and~\ref{thm:dynamic_opt_ef1}.

%\section{Practical implementation ideas*}
%\todo{just some preliminary considerations}
%
%We maintain a B+tree in which each node (internal and leaf) keys are compressed with Elias-Fano. In particular, each leaf holds $\rho m$ integers, while internal nodes $\rho b$, $1 \leq \rho \leq 2$. Block length $m$ and the optimal branching factor $b$ are to be determined experimentally.
%
%Each internal node holds:
%\begin{itemize}
%\item the number of currently stored keys \textsf{num\_keys};
%\item the maximum stored key \textsf{max\_key};
%\item an array \textsf{keys} of keys compressed with Elias-Fano;
%\item an array \textsf{children} of pointers to internal nodes representing node's children;
%\item an array \textsf{sizes} of integers representing the number of keys stored in the children: $\textsf{sizes}[i]=k$ means there are $k$ keys stored in the sub-tree rooted in the $i$-th child.
%\end{itemize}
%
%Each leaf holds:
%\begin{itemize}
%\item the number of currently stored keys \textsf{num\_keys};
%\item the maximum stored key \textsf{max\_key};
%\item an array \textsf{keys} of keys compressed with Elias-Fano.
%\end{itemize}
%
%$b$ and $m$ could be different, e.g. $m \geq b$, and not so big, for example $b=128$ and $m=256$. Since they are relatively small, the keys encoded with Elias-Fano are just operated via linear scan and re-encoded upon a merge/split and an insertion/deletion. The same holds for the sizes of each sub-tree.
%
%Fixing the universe of the leaf to one million, we can pack 64 integers in 1024 bits (2 cache misses). 64 integers take 4096 bits if represented with 8 bytes each ($4\times$ compression ratio).
%
%Leaves could be of 1024 ints compressed with EF and all the upper levels will take negligible space (1/1024). Each leaf could be further divided into small blocks of 128 ints at most. This division resembles the T structure, while the Btree the upper level made up of Y and P. For each block we keep its length (in 7 bits) and its lower bound.
%Overall we need 9 words: 8 for the lower bounds and 1 for the lengths (given that 1024/128 = 8 and 7$\times$8 = 56 bits). To find the proper block where we need to insert/delete/access, we just scan this level storing lengths and lower bounds.
%
%\parag{Remapping}
%At each level of the B+tree, the keys can be stored as the difference between original values and parent key value. This holds for all nodes except the left-most ones of each level. This strategy reduces the space taken by the keys compressed with Elias-Fano, but prevents from efficiently iterating through all the keys in the tree.
%
%\parag{Existing implementations}
%B-tree open source C++ implementation: \url{https://panthema.net/2007/stx-btree/}\\
%Fractal Tree Indexes (state-of-the-art for databases in practice): \url{https://github.com/Tokutek/ft-index}
%
%See also slides in \textsf{./fractal\_trees\_slides}.

==> related.tex <==
\section{Related work}\label{sec:related}

We organize the discussion of related work in three parts.
In the first part we describe the static Elias-Fano
representation because it is a key ingredient of our solutions.
Then we review the results concerning the static predecessor
and dynamic ordered set (and related) problems,
stressing what lower bounds
apply to these problems.
Recall that we use a RAM model with word size $w$ bits.

\subsection{Static Elias-Fano representation}\label{sec:ef}

\begin{lem}{\textup{Elias-Fano~\cite{Elias74,Fano71}.}}\label{lem:ef}
An ordered set $\seq \subseteq [m]$,
with $|\seq| = n$, can be represented in
$\ef(n,m) + o(n)$ bits
such that {\access} is supported in $O(1)$
and {\pred} in $O(1+\log(m/n))$,
where $\ef(n,m) \leq n\lceil\log(m/n)\rceil + 2n$.
\end{lem}

%\parag{Data structure and space analysis}
%\begin{proof}
\paragraph{Space complexity}
Let $\seq[i]$ indicate the $i$-th smallest of $\seq$.
We write each $\seq[i]$ in binary using $\lceil \log m \rceil$ bits.
The binary representation of each integer is then split into two parts:
a \emph{low} part consisting in the right-most
$\ell = \lceil \log(m/n)\rceil$ bits that we call \emph{low bits}
and a \emph{high} part consisting in the remaining $\lceil \log m \rceil - \ell$ bits that we similarly call \emph{high bits}.
Let us call $\ell_i$ and $h_i$ the values of low and high bits
of $\seq[i]$ respectively.
The integers $L = [\ell_0,\ldots,\ell_{n-1}]$ are written explicitly
in $n \lceil \log(m/n)\rceil$ bits and
they represent the encoding of the low parts.
Concerning the high bits, we represent them in \emph{negated unary}
using a bitmap of $n + 2^{\lfloor \log n \rfloor} \leq 2n$ bits as follows. We start from a $0$-valued bitmap $H$ and set the bit
in position $h_i + i$, for $i = 0,\ldots,n-1$.
It is easy to see that the $k$-th unary value of $H$, say $n_k$,
indicates that $n_k$ integers of $\seq$ have high bits equal to
$k$.
For example, if $H$ is $\{$1110, 1110, 10, 10, 110, 0, 10, 10$\}$
(as in Fig.~\ref{fig-ef}), we have that $H[1] = 1110$, so we know
that there are 3 integers in $\seq$ having high bits equal to 1.

Summing up the costs of high and low parts, we derive that Elias-Fano
takes $\ef(n,m) \leq n\lceil\log(m/n)\rceil + 2n$ bits.
Although we can opt for an arbitrary split into high and low parts,
ranging from $0$ to $\lceil \log m \rceil$,
it can be shown that $\ell = \lceil \log(m/n) \rceil$
minimizes the overall space of the encoding~\cite{Elias74}.
As explained in Section~\ref{sec:intro}, the space of Elias-Fano
is related to the information-theoretic minimum: it is
at most $1.56n$ bits redundant.

%Moreover, given that the information-theoretic lower bound is approximately $n \log_2 \frac{u}{n} + n\log_2 e$ bits,
%it can be shown~\cite{Elias74} that less than half a bit is wasted per element by Formula~\ref{ef_space}.

\begin{figure}
\centering
\includegraphics[scale = 0.8]{{{figures/ef}}}
\caption{An example of Elias-Fano encoding.
The missing 3-bit configuration 101 is highlighted in bold.
}
\label{fig-ef}
\end{figure}

\paragraph{Example}
Fig.~\ref{fig-ef} shows a graphical example for the sorted
set $\seq$ $=$ $[$3, 4, 7, 13, 14, 15, 21, 25, 36, 38, 54, 62$]$.
The \emph{missing high bits} embody the representation of the fact that using $\lfloor \log_2 n \rfloor$ bits to represent the high part of an integer, we have \emph{at most} $2^{\lfloor \log_2 n \rfloor}$ distinct high parts because not all of them could be present. In Fig.~\ref{fig-ef}, we have $\lfloor \log_2 12 \rfloor = 3$ and we can form up to $8$ distinct high parts. Notice that, for example, no integer has high part equal to 101 which are, therefore, ``missing'' high bits.

%\parag{Random access}
\paragraph{Random access}
A remarkable property of Elias-Fano is that it can be \emph{indexed}
to support {\access} in $O(1)$ worst-case.
The operation is implemented by building an auxiliary data structure
on top of $H$ that answers $\select_1$ queries.
The answer to a $\select_b(i)$ query over a
bitmap is the
position of the $i$-th bit set to $b$.
This auxiliary data structure is \emph{succinct} in the sense that it is negligibly small in asymptotic terms, compared to $\ef(n,m)$,
requiring only $o(n)$ additional bits~\citep{MN07,Vigna13},
hence bringing the total space of the encoding to $\ef(n,m) + o(n)$ bits.
For a given $i \in [0,n)$, we proceed as follows.
The low bits $\ell_i$ are trivially retrieved as
$L[i\ell, (i + 1)\ell)$.
The retrieval of the high bits is, instead, more
complicated.
Since we write in negated unary how many integers share the same high part,
we have a \textbf{1} bit for every integer in $\seq$
and a \textbf{0} for every distinct high part.
Therefore, to retrieve $h_i$, we need to know how many \textbf{0}s
are present in $H[0, \select_1(i))$.
This quantity is evaluated on $H$ in $O(1)$ as $\select_1(i)-i$.
Lastly, re-linking the high and low bits together is as simple as:
$\access(i) = ((\select_1(i)-i) << \ell) \mid \ell_i$, where $<<$ indicates the left shift operator and $\mid$ is the bitwise OR.

%\parag{Predecessor query}
\paragraph{Predecessor search}
The query $\pred(x)$ is supported in $O(1+\log(m/n))$ time as follows.
Let $h_x$ be the high bits of $x$. Then for $h_x > 0$, $i = \select_0(h_x) - h_x + 1$ indicates that there are $i$ integers in $S$ whose high bits are less than $h_x$. On the other hand, $j = \select_0(h_x + 1) - h_x$ gives us the position at which the elements having high bits larger than $h_x$ start. The corner case $h_x = 0$ is handled by setting $i = 0$.
These two preliminary operations take $O(1)$.
Now we can conclude the search in the range $\seq[i,j]$, having \emph{skipped} a potentially large range of elements that, otherwise, would have required to be compared with $x$.
The range may contain up
to $u/n$ integers that we search with binary search.
The time bound follows.
In particular, it could be that $\pred(x) < \seq[i]$:
in this case $\seq[i - 1]$ is the element to return if $i > 0$.
%\end{proof}

%As an example, consider the query $\suc(30)$
%over the sequence illustrated in Fig.~\ref{fig-ef}.
%Since $h_{30} = 3$, we have $i = \select_0(3) - 3 + 1 = 7$ and $j = \select_0(4) - 3 = 8$. Therefore we conclude our search in the range $\seq[7,8]$ by returning $\suc(30) = \seq[8] = 36$.

%In the specific context of inverted indexes, the
%query {\suc} is called {\Nextgeq} (Next Greater-than or Equal-to).

\paragraph{Partitioning the representation}
In this article we will use extensively the following
property of Elias-Fano.

\begin{prop}\label{prop:almost_convexity}
Given an ordered set $\seq \subseteq \{0,\ldots,m\}$,
with $|\seq| = n$, let $\ef(\seq[i,j))$
indicate the Elias-Fano representation of $\seq[i,j)$,
for any $0 \leq i < j \leq n$.
Then given an index $k \in [1,n)$,
we have that $\ef(\seq[0,k)) + \ef(\seq^{\prime}[k,n)) \leq \ef(\seq[0,n))$,
where $\seq^{\prime}[l] = \seq[l]-\seq[k-1]+1$, for $l = k,\ldots,n-1$.
\end{prop}

The property tells us that splitting the Elias-Fano encoding of $\seq$
does not increase its space of representation.
This is possible because each segment can be encoded
with a \emph{reduced universe}, by subtracting to each integer
the last value of the preceding segment (the first segment is left
as it is).
Informally, we say that a segment is ``re-mapped'' relatively
to its own universe.
The property can be easily extended to work with an arbitrary number of splits. Let us now prove it.

\begin{proof}
We know that $\ef(\seq[0,n))$ takes $n\phi + n + \lceil m/2^{\phi} \rceil$ bits, where $\phi = \lceil \log(m/n) \rceil$.
Similarly, $\ef(\seq[0,k)) = k\phi_1 + k + \lceil m_1/2^{\phi_1} \rceil$
and $\ef(\seq^{\prime}[k,j)) = (n-k)\phi_2 + (n-k) + \lceil m_2/2^{\phi_2} \rceil$, where $m_1 = \seq[k-1]$ and $m_2 = \seq[n-1] - m_1 + 1$,
are minimized by choosing
$\phi_1 = \lceil \log(m_1/k)\rceil$ and $\phi_2 = \lceil \log(m_2/(n-k))\rceil$.
Any other choice of $\phi_1$ and $\phi_2$ yields a larger cost, therefore:
$\ef(\seq[0,k)) + \ef(\seq[k,n))$ $\leq$ $k\phi + (n-k)\phi + k + (n-k) + \lceil m_1/2^{\phi} \rceil + \lceil m_2/2^{\phi} \rceil$ $\leq$ $n\phi + n + \lceil m/2^{\phi}\rceil$ $=$ $\ef(\seq[0,n))$.
\end{proof}

An important consideration to make is that Property~\ref{prop:almost_convexity}
needs the knowledge of the value $\seq[k-1]$ to work
--- the pivoting element ---
which can be stored in $O(\log m)$ bits.
This means that for small values of $n$ it can happen that the
space reduction does \emph{not} exceed $O(\log m)$ bits.
Since we do not deal with such values of $n$, we
always assume that this is not the case.

\subsection{The static predecessor problem}\label{sec:pred}
There are two obvious solutions
to the static predecessor problem.
The first uses an array $P[0..m)$ where we store the answers
to all possible queries. In this case $\pred(x) = P[x]$ for any
$x < m$ ($P[0] = -\infty$), thus
the problem is solved in $O(1)$ worst-case time
and $O(m \log m)$ bits.
The second solution stores $\seq$ as a sorted array and answers
the queries using binary search, therefore taking $O(n \log m)$ bits
and $O(\log n)$ worst-case time.
Both solutions are unsatisfactory: the first one because of its
space; the second one because of its time.
%Therefore, in the following we assume to have a polynomial space budget,
%i.e., $O(n^{\Theta(1)})$ memory words.

\return
\citet*{Ajtai88} proved the first $\omega(1)$-time lower bound
for polynomial space, i.e., $O(n^{\Theta(1)})$ memory words,
claiming that $\forall \, w$, $\exists \, n$
that gives $\Omega(\sqrt{\log w})$ query time.
For the \emph{dense} case of $m = n (\log n)^{O(1)}$,
~\citet*{pagh2001low} gave a static data structure
taking $B + o(n)$ bits and
answering membership and predecessor queries in $O(1)$ worst-case time.
(We consider larger universes in this article.)
~\citet*{BF99,BF02} proved two strong bounds for any {cell-probe} data structure.
%\footnote{In the cell-probe computational model, described by~\citet*{Yao81}, computation is for free given that we only take into account \emph{word reads}. It is not a very realistic model of computation, but it is useful to prove lower bounds because it is a stronger model than RAM and trans-dichotomous RAM.}
They proved that $\forall \, w$, $\exists \, n$ that requires
$\Omega(\log w / \log\log w)$ query time and that $\forall \, n$, $\exists \, w$ that requires $\Omega(\sqrt{\log n / \log\log n})$ query time.
They also gave a static data structure achieving $\Oh(\min\{\log w / \log\log w, \sqrt{\log n / \log\log n}\})$ which is, therefore, optimal.

\return
Building on a long line of research,~\citet*{PT06,PT07} finally proved the following optimal (up to constant factors) space/time trade-off.

\begin{thm}{\textup{\citet*{PT06,PT07}.}}\label{thm:pred}
A static data structure representing $n$ integer keys in $z$ bits,
takes time
$$
\Theta\Big(\min\Big\{\frac{\log n}{\log w}, \log \frac{w - \log n}{a}, \frac{\log(w/a)}{\log ( \frac{a}{\log n} \log(w/a) )}, \frac{\log(w/a)}{\log ( \log(w/a) / \log \frac{\log n}{a} )} \Big\}\Big)
$$
to answer a {\pred} query, where $a = \log(z/n)$.
\end{thm}

% \emph{optimal} space/time trade-off for a \emph{static} data structure taking $z$ bits of space, with
%%$a$ being the number of bits necessary to represent the mean number of bits per integer, i.e.,
%$a = \log\frac{m}{n} - \log w$
%\begin{align}\label{eq:PTlowerbound}
%\Theta\Big(\min\Big\{\log_w n, \log \frac{w - \log n}{a}, \frac{\log \frac{w}{a}}{\log ( \frac{a}{\log n} \log \frac{w}{a} )}, \frac{\log \frac{w}{a}}{\log ( \log \frac{w}{a} / \log \frac{\log n}{a} )} \Big\}\Big)
%\end{align}

This lower bound holds for cell-probe, RAM, trans-dichotomous RAM,
external memory and communication game models.
The first branch of the trade-off indicates that, whenever one integer
fits in one memory word, fusion trees~\cite{FW93} are optimal as they
have $O(\log n / \log w)$ query time.
The second branch holds for {polynomial universes},
i.e., when $m = n^\gamma$, for any $\gamma = \Theta(1)$.
In such case we have that $w = \Theta(\log m) = \Theta(\log n)$,
therefore $y$-fast tries~\cite{Willard83} and van Emde Boas trees~\cite{Boas75,Boas77,BKZ77} are optimal with query time $O(\log\log n)$.
We focus on these two branches in this work.
The last two bounds of the trade-off, instead, treat the case for \emph{super-polynomial} universes
and are out of scope for this work.
% In particular, the third branch matches the lower bound by~\citet*{BF99,BF02} that requires $O(n^{\Theta(1)})$
%words of space. The fourth branch improves the latter space occupancy, showing that $n^{1 + 1/\exp(\log^{1-\epsilon}\log m)}$ words are sufficient for any $\epsilon > 0$.

%By tuning the parameter $a$ in (\ref{eq:PTlowerbound}), we can obtain different space/time trade-offs, as we will show in Section~\ref{sec:static_ef_opt_succ}.

%As an example, suppose we want $\Oh(n \polylg n)$ words. With such space budget, we have that $a$ becomes $\Oh(\log\log n)$ and (\ref{eq:PTlowerbound}) reduces to $\Theta\Big(\min\Big\{  \log_w n, \frac{\log w}{\log (\log w / (\log w / \log\log n))} \Big\}\Big)$.
%This shows that $y$-fast tries and van Emde Boas trees are optimal whenever $w = \Oh(\polylg n)$ and fusion trees are optimal whenever $\log w = \Omega(\sqrt{\log n} \log\log n)$.

%\citet*{GHSV07} gave a static data structure representing a set of $n$ integers taking $gap + \Oh(n \log(u/n)/\log n) + \Oh(n \log\log(u/n))$ bits while supporting $rank$ in nearly optimal time $$\Oh\Big(\min\Big\{\sqrt{\frac{\log n}{\log\log n}}, \log\log n \frac{\log w}{\log\log w}, \log\log n +\frac{\log n}{\log w}\Big\}\Big)$$ and $\select$ in $\Oh(\log\log n)$ time. Their data structure eliminates the $o(u)$ term of previous work~\cite{MN07,SG06}.

\subsection{Dynamic problems}\label{sec:dynamic_problems}
%We now review the results concerning the maintenance of a
%\emph{dynamic} set of integer keys.
%We will reuse some of these results later on in this article.

As far as the {\access} operation is \emph{not} supported,
the following results hold.
The van Emde Boas tree~\cite{Boas75,Boas77,BKZ77} is a recursive data structure that maintains $\seq$ in $O(m \log m)$ bits
and $O(\log w)$ worst-case time.
\citet*{Willard83} improved the space bound to $O(n \log m)$ bits
with the $y$-fast trie. (The bound for {\ins}/{\del} is amortized
rather than worst-case).
When polynomial universes are considered,
~\citet*{PT06} proved that
van Emde Boas trees and $y$-fast tries
have an optimal query time
for the dynamic predecessor problem too,
that is $O(\log\log n)$ worst-case.

Extending their result to the dynamic predecessor problem,
\citet*{BF99,BF02} proved that any cell-probe data structure
using $(\log m)^{O(1)}$ bits per memory cell and $n^{O(1)}$ worst-case time for insertions, requires $\Omega(\sqrt{\log n / \log\log n})$
worst-case query time.
They also proved that, under a RAM model,
the dynamic predecessor problem can be solved
in $O(\min\{\log\log n \log w / \log\log w$, $\sqrt{\log n / \log\log n}\})$,
using linear space.
This bound was matched by~\citet*{AT07} with the so-called
\emph{exponential search tree}.
This data structure has an optimal bound of $O(\sqrt{\log n / \log\log n})$ worst-case time for searching and updating $\seq$, using polynomial space.

%They support an \key{extended} $\search$ operation (checking whether a key is present or not in the dictionary is called \textsf{lookup}).
%More specifically they support $\minimum$, $\maximum$, $\suc$, $\pred$ and $\del$ in $\Oh(1)$ and only do $\ins$ and $\search$ in $\Theta(\sqrt{\log n / \log\log n})$ time.
%They also support \key{finger searches} in optimal $\Oh(\sqrt{\log d / \log\log d})$, where $d$ is the absolute distance between the two keys, and \key{finger updates} in $\Oh(1)$.

\return
The lower bound for the problem changes
by considering the {\access} operation
because this operation is related to the
\emph{partial sums problem} that is,
given an integer array $A[0..n)$,
support $\sm(i)$ returning the sum of the
first $i+1$ integers,
$\upd(i,\Delta)$ which sets $A[i]$ to $A[i] + \Delta$
and $\search(x)$ which returns the index
$i \in [0,n)$ such that $\sm(i) < x \leq \sm(i+1)$.
~\citet*{FS89}
proved a bound of
$\Omega(\log n / \log\log n)$
amortized time for this problem
(see also the extended version of the article by~\citet*{PT14} --- Section 5).
Therefore, this is the lower bound that applies to our
problem as well.
\citet{BCGSVV15} extended the problem as to also support dynamic
changes to the array.%, thus obtaining the following result.

%combined the static solution of~\citet*{DP04}
%with the one by~\citet*{PT14} to solve the \emph{dynamic}
%partial sums problem
%over an array of size $n$.
%
%in optimal $O(\log n / \log (w / \delta))$ time
%per operation and linear space,
%where $\delta$ is the number of bits needed to encode
%the quantity that we sum to the elements of the array.

%\begin{lem}{\textup{\citet{BCGSVV15}}}\label{lem:dps}
%The dynamic prefix sums problem, over an array of size $n$
%storing $w$-bit integers,
%can be solved in linear space and optimal $O(\log n / \log(w/\delta))$
%time per operation for a given parameter $\delta > \log \Delta$.
%\end{lem}


\citet*{FS89} also proved that $\Omega(\log n / \log\log n)$
amortized is necessary
for the \emph{list representation problem}, that
is to support {\access}/{\ins}/{\del}.
However, this
problem is slightly different than the one tackled here,
because one can specify the \emph{position} of insertion of a key.
Likewise, the {\del} operation specify the position of the key,
rather than the key itself.
%Their lower bound does not apply to dynamic predecessor queries and holds for the cell-probe computational model~\cite{Yao81}.
\citet*{RRR01} also addressed the list representation problem
(referred to as the \emph{dynamic array problem})
and provide two solutions.
The first solution is given by the following lemma.

\begin{lem}{\textup{\citet*{RRR01}.}}\label{lem:dynamic_array}
% solution 1
A dynamic array containing $n$ elements
can be implemented to support {\access} in $O(1)$,
and {\ins}/{\del} in $O(n^{\epsilon})$ time
using $O(n^{1-\epsilon})$ pointers,
where $\epsilon$
is any fixed positive constant.
% solution 2
%A dynamic array containing $n$ elements
%can be implemented using $o(n)$ bits of redundancy
%and supporting {\access}, {\ins} and {\del}
%in $O(\log n / \log\log n)$ amortized time.
\end{lem}

The second solution supports all the three operations
in $O(\log n / \log\log n)$ amortized time.
Both solutions take $o(n)$ bits of redundancy
(besides the space needed to store the array)
and the time bounds are optimal.

\return
\citet*{FW93} solved that dynamic predecessor problem in
$O(\log n / \log\log m)$ time and $O(n)$ space
with the fusion tree.
This data structure is a $B$-tree with branching factor
$B = w^{O(1)}$ that stores in each internal node a \emph{fusion node}
a small data structure able of answering predecessor queries in $O(1)$
for sets up to $B$ integers.
It takes, however, $O(B^4)$ time to construct and update a fusion node.
~\citet*{PT14} showed that it is possible
to ``dynamize'' the fusion node and obtained the following result.

%\begin{lem}{\textup{\citet*{PT14}.}}\label{lem:small_sets}
%A dynamic set of $w^{O(1)}$ $b$-bit integers
%can be implemented with $O(wb)$ bits and
%supporting
%{\ins}, {\del}, {\rank}, {\select} and {\pred}
%in $O(1)$ per operation.
%\end{lem}
%
%Using such lemma, they used a standard reduction by~\citet*{Willard00}
%to obtain a solution working for arbitrary set sizes.
%
%\begin{lem}{\textup{\citet*{Willard00}}}\label{lem:willard}
%A $B$-tree with out-degree $B$, height $h$ and storing
%the data in the leaves,
%can be maintained in $O(h)$ worst-case time if:
%searches, insertions and deletions take $O(1)$ time per node when no splits or merges occur, and
%merging or splitting a node of size $B$ requires $O(B)$ time.
%\end{lem}

\begin{lem}{\textup{\citet*{PT14}.}}\label{lem:optimal_dynamic_sets}
An ordered set $\seq \subseteq [m]$,
with $|\seq| = n$, can be represented in
$O(n \log m)$ bits and supporting
{\ins}, {\del}, {\rank}, {\select} and {\pred}
in $O(\log n / \log\log m)$ per operation.
\end{lem}

The time bound of $O(\log n / \log\log m)$ is optimal, matching
a lower bound by~\citet*{FS89} for dynamic ranking and selection,
and that of predecessor queries for non-polynomial universes
(first branch of the trade-off from Theorem~\ref{thm:pred}).

%In fact note that, in this case,
%$\log\log n$ is asymptotically less than $\log n / \log\log n$.

%The resizeable array of~\citet*{BCDMS99} supports $\ins$ and $\del$ of elements at both ends of the array and $\access$ in constant time. The data structure uses $\Oh(\sqrt{n})$ words of extra space, where $n$ is the current size of the array. Insertions/deletions in middle positions of the array are not supported.

%\parag{Other results}

%We conclude this section by mentioning some additional results,
%that will be useful in the following.


%Though not devised for integer sets, the \emph{extended CRAM} (Compressed Random Access Memory) data structure described by~\citet*{JSS12} allows a string $\seq$ of length $n$ to be stored using its $k$-th order empirical entropy, $nH_k(\seq)$, plus a redundancy of $\Oh(n\log\sigma(k\log\sigma + (k+1)\log\log n)/\log n)$ bits for every $0 \leq k < \log_{\sigma}n$, where $\sigma$ is the size of the alphabet.
%Insertions/deletions of characters and random access to any consecutive $\log_{\sigma}n$ bits are all supported in optimal $O(\log n / \log\log n)$ worst-case time.
%We will exploit the part of this work dedicated to the memory management (Appendix A).
%(\citet{GRRV13} improved the previous space bound by using $nH_k(\seq) + O(n \log\log n / \log_{\sigma} n)$ bits and maintaining the asymptotic optimality for all operations.)

%\citet*{NN13} gave a data structure supporting {\access}, {\rank}
%and {\select} queries over a string $\seq$, as well as insertions/deletions of symbols, in optimal $O(\log n / \log\log n)$ time and taking
%$nH_0(\seq) + O(n + \sigma(\log \sigma + (\log n)^{1+\epsilon}))$ bits of space, for any constant $0 < \epsilon < 1$.
%Of particular interest for our purposes, is the data structure described in Appendix A.1 concerning the organization of data in small blocks.
%The high-level idea is to maintain a tree of constant height with node degree $\log^\delta n$, for some $0 < \delta < 1$, and leaves containing $o(\log n)$ elements each. As each internal node can fit in one machine word, the tree supports basic search operations in $O(1)$ time by using a small pre-computed table.
%In order to handle small blocks of sorted integers, we will make use of a similar data structure in Section~\ref{sec:dynamic}.
